A Model-based Projection Technique for Segmenting Customers

We consider the problem of segmenting a large population of customers into non-overlapping groups with similar preferences, using diverse preference observations such as purchases, ratings, clicks, etc. over subsets of items. We focus on the setting where the universe of items is large (ranging from thousands to millions) and unstructured (lacking well-defined attributes) and each customer provides observations for only a few items. These data characteristics limit the applicability of existing techniques in marketing and machine learning. To overcome these limitations, we propose a model-based projection technique, which transforms the diverse set of observations into a more comparable scale and deals with missing data by projecting the transformed data onto a low-dimensional space. We then cluster the projected data to obtain the customer segments. Theoretically, we derive precise necessary and sufficient conditions that guarantee asymptotic recovery of the true customer segments. Empirically, we demonstrate the speed and performance of our method in two real-world case studies: (a) 84% improvement in the accuracy of new movie recommendations on the MovieLens data set and (b) 6% improvement in the performance of similar item recommendations algorithm on an offline dataset at eBay. We show that our method outperforms standard latent-class and demographic-based techniques.

==> 1.1_related_work.tex <==
%!TEX root = CustPrefSegment.tex

\subsection{Relevant literature} 
\label{sec:related_work}

Our work has connections to the areas of marketing and machine learning. Segmentation is a classical marketing problem, and existing literature has proposed a broad array of latent class models (with either finite or infinite number of classes), each appropriate for specific application contexts. 
%In the context of these models, the work has broadly focused on segmentation methodologies based on general-purpose clustering techniques (such as $k$-means, agglomerative/hierarchical clustering, etc.), the EM algorithm, and other Bayesian techniques. 
Our work is complementary to this literature since we can leverage the domain knowledge used in specifying customized models of customer behavior and preferences in different contexts in our model-based projection technique.
%These general purpose techniques, however, lack guarantees on statistical efficiency and can be shown to converge to incorrect or suboptimal segmentations~\citep{kannan2005spectral}. 
On the other hand, the literature in machine learning has focused on general-purpose methodologies with strong theoretical guarantees to carry out clustering. However, these algorithms do not readily apply when observations are categorical and/or have missing entries, typical in settings of interest to marketing. 
%Further, the theoretical guarantees do not apply to the modeling structures considered in the marketing literature. 
Our work addresses these gaps in the literature. We first summarize the relevant work in the marketing literature and then discuss the methodological connections to the work in machine learning. Due to space constraints, we keep the discussion succinct and refer the reader to Appendix~\ref{app:relwork} for a more detailed description and additional references.

{\bf Marketing.} There has been a wide variety of segmentation techniques proposed in the marketing literature (refer to~\citet{wedel2012market} for a comprehensive overview), however since ours is a methodology paper, we find it most useful to compare against techniques (or algorithms) employed to perform segmentation of customers. Broadly, these techniques fall into two classes: {\em distance- or similarity-based} which define suitable distance metrics between customers and then group the customers into clusters based on these distances, and {\em model-based} which associate customer observations with well-defined probabilistic models. Because our approach relies on some probabilistic model of customer behavior, we review the model-based techniques below (see~\citep{jain2010data} for a review of distance- or similarity-based techniques).

% We review both these techniques in detail below:

% {\bf Distance/Similarity-based Techniques}. The goal of such techniques is to separate the customers into different segments using suitably-defined similarity between any pair of customers. Some of the popular techniques include k-means, Kohonen's Self-Organizing Map (SOM)~\citep{kohonen1998self} and agglomerative/hierarchical clustering (see~\citep{punj1983cluster, dolnicar2003using} for a review of these techniques).  The method has been widely used for doing cluster analysis in a number of different domains including travel and tourism~\citep{arimond2001clustering}, sport participation~\citep{harwood2004motivational}, online game industry~\citep{lee2004cross} as well as food preferences~\citep{honkanen2004preference}. However, most oft hese works either ignore observations with missing data or have some adhoc mechanism to impute them (refer to section~\ref{sec:intro} for generic issues with similarity-based methods). Our contribution in this paper is a {\em new} clustering technique that can principally handle missing data, while retaining some nice properties of similarity-based methods.%Most of the clustering techniques only focus on optimizing similarity within each segment and generally ignore relationships between segmentation descriptive variables and exogenous response variable(s). As a result it lacks predictability of segment response to variables of interest such as brand preferences, and therefore more predictive approaches were sought for.
%However, conjoint analysis studies typically assume some model of customer preferencechoice behavior (e.g. Multinomial Logit Model) and then estimate the parameters based on the observed data.
%As a result they are sensitive to model misfit and other issues highlighted in section~\ref{sec:intro}. Further, because of the strain on the respondents, the number of products/attributes that can be used in a conjoint study are limited. Our approach tries to overcome some of these issues by proposing a more robust clustering technique.

% {\bf Model-based Techniques}. 
The model-based approaches, in turn, can be categorized into two types:
%Our work has rich connections to the literature in Statistics/Machine Learning as well as Marketing. Existing work in Statistics/Machine Learning has studied the problem of clustering, with a plethora of techniques that are mostly agnostic to the underlying application (or domain) at hand. Literature in marketing, on the other hand, has focused on application-driven techniques for segmentation.
%
%Clustering is defined as the problem of partitioning data objects into groups, such that objects in the same group are similar, while objects in different groups
%are dissimilar (see~\citep{jain1988algorithms} and~\citep{jain1999data} for a review). As discussed in the introduction, there are two broad classes of clustering techniques - {\em model-free} and {\em model-based}. Most of the model-based clustering techniques are based on finite mixture models~\citep{mclachlan2004finite} and have shown promising results in a corpus of domains. Gaussian Mixture Models (GMMs) are by far the most extensively used for continuous data, with applications ranging from separating diabetic and normal subjects~\citep{symons1981clustering}, classifying astronomical data~\citep{celeux1995gaussian}, and clustering gene expressions~\citep{yeung2001model}. Multinomial models have been successfully used for high-dimensional text clustering applications~\citep{meilua2001experimental}. For clustering more complex data such as time sequences, the dominant models have been Markov chains~\citep{ramoni2002bayesian} and Hidden Markov Models (HMMs)~\citep{smyth1997clustering}.~\citep{cadez2000general} present a unifying probabilistic framework for clustering individuals or systems into groups for non-vector data such as time series, trajectories etc. using the Expectation-Maximization algorithm. Compared to similarity-based (or model-free) methods,
%model-based methods offer better interpretability since the resulting model for each cluster directly characterizes that cluster. However, as alluded to earlier, these methods require specification of the model type {\em a priori} and therefore, are sensitive to model misfit. Further, these methods try to learn the generative model of data for each cluster, which in some sense is an ``overkill'' if all we are interested in is clustering customers. Our work borrows the statistical framework of model-based clustering but leverages this observation to propose a clustering algorithm that can overcome some of the disadvantages of model-based approaches (see section~\ref{sec:intro}).
latent class analysis and continuous distribution models. Latent class analysis imposes a discrete model of heterogeneity where it is assumed that the market is partitioned into (discrete) customer segments. The observed data are then used to compute segment-level membership for each customer. This approach was pioneered by~\citet{kamakura1989probabilistic} who propose a probabilistic choice model to segment households based on brand preferences and price sensitivities. This was extended by~\citet{gupta1994using} who incorporated demographic variables and~\citet{kamakura1996modeling} who incorporated differences in customer choice-making processes.
%who demonstrate that using information on demographic variables in addition to purchase histories leads to a better delineation of segments. This was further generalized by~\citet{kamakura1996modeling} who  into an integrated model of customer heterogeneity. 
%They proposed a finite mixture of nested-logit models that simultaneously identifies consumer segments on the basis of their preferences, response to the marketing mix, and choice processes. 
%In the context of preference-based segmentation,~\citet{desarbo1992latent} used ratings-based conjoint data and~\citet{desarbo1995market} used choice-based conjoint data to segment markets using a latent class approach.
%Their integrated provides managers with a more complete portrait of brand preferences, choice process, and price/promotion response within each consumer segment, and is a generalization of the model proposed in~\citep{kamakura1989probabilistic}.
%In particular, their approach allows for multiple choice processes across segments, and empirical evaluation on household scanner data resulted in 8 segments that differ in their preferences for brands and product forms. 
%All of these approaches share the same pitfalls as that of (finite) mixture models (see section~\ref{sec:intro}). In addition, the number of identified segments were always less than 10 which shows that it is harder to obtain a larger number of segments with the latent class approach. Our technique can incorporate a priori models of customer behavior, but can also infer it in a data-driven fashion, making it more robust to model misspecification. Further, as will become clearer in section~\ref{sec:setup}, we only estimate the population-level model and can therefore recover a larger number of underlying segments while achieving significant improvements in running times.
%
%Further, they usually take into account product (or item) features and attributes like brand, price, display etc., whereas we focus only on customer features for the purposes of segmentation. Refer to~\citep{wedel2012market} for more references. 
%in many fields within marketing, emphasis should be on individual customer contact and direct marketing approaches, and therefore individual-level response parameters are required. 
One issue with the latent class approach is the discrete model of heterogeneity and it has been argued~\citep{allenby1998heterogeneity,wedel1999discrete} that individual-level response parameters are required for direct marketing approaches. As a result, continuous mixing distributions have been proposed that capture fine-grained customer heterogeneity, leading to hierarchical Bayesian estimation of models~\citep{allenby1995using,rossi1996value,allenby1998marketing}.

However, both latent class analysis and continuous distribution model approaches are usually estimated on data from small samples of customers each with many repeated observations, with the primary aim of understanding the customer heterogeneity and running counterfactual analyses. Further, they usually assume access to complete well-defined features for customers and/or observations (such as demographics, product attributes, etc.), which in many cases is unavailable. Consequently, they do not scale when the goal is to segment an entire population of customers and there are many missing observations. Our algorithm is explicitly designed to handle observations with missing entries and can be applied even when the data is less-structured or even unstructured (refer to the case study in Section~\ref{sec:ebay}).
%Our focus in this paper is to explicitly partition the customer population into segments---we overcome these limitations since we do not estimate coefficients for each segment (or individual customer), instead we just compute a single estimate by pooling all the data, allowing us to estimate complex models, and making our approach fast and scalable.

%More recently, there have been many works that use customer segmentation in specific applications.~\citep{manchanda1999shopping} develop a framework for investigating
%multicategory purchase decisions in the grocery shopping context using a Hierarchical Bayes model.~\citep{ansari2003customization} use clickstream data from users to develop a statistical approach for customization of information on the Internet. The authors apply the model to the context of permission-based e-mail marketing, and show that their method increases the expected number of click-throughs by 62\%.~\citep{boxall2002understanding} apply the latent segmentation approach to wilderness recreation park choice data and showed that hypothetical policy changes had a considerably different welfare effect than a standard single segment model that does not account for heterogeneity.
%~\citep{chung2003general} use mixture distributions in a hierarchical Bayesian framework to incorporate customer heterogeneity for modeling bundling choices. Using students' purchase decisions for a bundle of a monitor, computer and printer, they show that their approach can identify market segments, estimate individual reservation prices for bundles and determine the optional bundle prices for different segments.~\citep{bhatnagar2004segmenting} develop a utility-based model to examine how customer preferences are shaped by the (perceived) risks and benefits of online shopping. They segment the customers based on their sensitivity to the benefits and risks of Internet shopping and calibrate their model on survey data.~\citep{castro2007influence} explores the influence of a psychographic feature of tourists, viz. need for variety, as a latent base for segmentation. They conduct a latent class analysis and evaluate the effect of the `image' of a destination on the future behavior of tourists.

{\bf Machine learning.} The literature in machine learning on the use of mixture models for clustering is vast~\citep{mclachlan2004finite}. Several advances have been made in the the last two decades in developing techniques with strong theoretical guarantees to recover the underlying components given a collection of samples generated from the mixture distribution. 
%The general setting considered is as follows. There is an underlying mixture of distributions described by the collection $\set{D_1, \dotsc, D_K}$ and associated mixing weights $\set{q_1, \dotsc, q_K}$ such that $\sum_{k=1}^K q_k = 1$ and $q_k \geq 0$ for all $k$. We are given $m$ samples from this mixture with each sample generated by choosing the mixture component $k$ with probability $q_k$ and then choosing a sample from the distribution $D_k$. The objective is to correctly classify ``most'' of the samples into their corresponding components. 
Our model-based projection algorithm draws inspiration from spectral projection techniques for learning mixtures of $K$ multivariate Gaussians~\citep{vempala2004spectral,achlioptas2005spectral,kannan2005spectral}. These techniques rely on projecting the samples onto the $K$-dimensional subspace spanned by the top-$K$ right singular vectors of the sample matrix (matrix consisting of each sample as a row vector) i.e., its $K$ principal components. The projections are then clustered using distance-based classification techniques. The lower-dimensional projections of the samples are more tightly concentrated (due to averaging) around the projections of the respective mean vectors. In addition, choosing the subspace spanned by $K$ principal components of the sample matrix ensures that the distance between the mean vectors is preserved so that as long as the mean vectors were ``well-separated'' in the original space, we can recover the mixture components.
%As a result, separation that scales only in the lower-dimension $K$ is sufficient to ensure recovery of the segments. 
%The first provable results for learning mixtures of Gaussians is due to~\citet{dasgupta1999learning}, who showed that random projections can be used to learn mixtures of spherical Gaussians, with standard deviation $\sigma$, provided the {\em separation} (the Euclidean distance) between any pair of mean vectors is at least $O(\sigma \sqrt{n})$. This was generalized to non-spherical Gaussians by~\citet{sanjeev2001learning}. However, because of the dependence on the dimension $n$, these techniques were not scalable to high dimensional spaces.
%%Shortly after,~\citet{dasgupta2000two} proposed an EM-based algorithm and showed that it works with a smaller separation of $O(\sigma n^{1/4})$ between the mean vectors.~\citet{sanjeev2001learning} generalized this result to non-spherical Gaussians.
%~\cite{vempala2002spectral} were the first to remove the dependence of the separation on the dimension $n$. They proposed a spectral algorithm and showed that it recovers spherical Gaussians with $O(\sigma K^{1/4})$ separation, where $K$ is the number of mixture components. 
%
%Recent work has focused on recovering mixtures of more general distributions.~\cite{kannan2005spectral} and~\cite{achlioptas2005spectral} extend the results of~\citep{vempala2004spectral} to recover mixtures of general log-concave distributions (i.e., the log of the density function is concave).~\cite{chaudhuri2008learning} focus on the problem of recovering mixtures of product distributions and propose a ``multi-view'' method, which can recover the mixture components when the separation scales logarithmically in skewed mixing weights.

%More recently, method-of-moment based techniques, with stronger theoretical guarantees have been proposed. These methods rely on computing lower-order moments from the samples, specifically, the second and third order moments. These moments are used to derive a symmetric tensor, and the problem of estimating model parameters is reduced to extracting an orthogonal decomposition of the symmetric tensor.~\cite{anandkumar2014tensor} show that for a broad class of mixture models -- which includes mixtures of Gaussians and Hidden Markov models -- the tensors possess special structures so that the decomposition can be done efficiently.~\cite{hsu2013learning} show that mixtures of spherical Gaussians can be recovered without the need for any separation requirements, provided some non-degeneracy conditions are satisfied.
Our work deviates from the above body of work in the following ways. First, we focus on the setting in which the observations are categorical and have (many) missing entries, as opposed to existing work, which mostly focuses on the case when the observations are vectors of real numbers, with no missing entries. Second, most of the theoretical guarantees in the above literature focus on the regime when the dimension $n$ is fixed, but the number of samples $m$ is large. However, it is more natural in our case to consider a fixed population size $m$ of customers and allow the number of observations $n$ to grow. Our theoretical development (see Section~\ref{sec:results}) focuses precisely on this setting, for any (fixed) population size $m$ that is large enough.

In addition, the {\em project} step in our segmentation algorithm has connections to matrix factorization techniques in collaborative filtering applications~\citep{rennie2005fast,mnih2007probabilistic,koren2009matrix}, where the user-item rating matrix is factorized as a product of two low-rank matrices---one specifying the user representation and the other an item representation, in a lower dimensional space. Our approach can be viewed as a generalized matrix factorization--- specifically, instead of treating all the items together and working with the raw observations (such as 1-5 star ratings), our technique identifies subsets of items that are most similar (such as movies with same genres or products in the same category), transforms observations in each subset independently, and then applies matrix factorization to the transformed matrix (refer to Section~\ref{sec:item_cat} for more details).

%Third, most of the existing work assumes that the observed samples have no missing entries. \ashwin{While the algorithms (such as spectral decomposition) can, in principle, be extended to cases with missing entries, such extensions essentially involve performing ad hoc imputations, by imposing general-purpose structures (such as the sample matrix being low-rank); see~\cite{mnih2007probabilistic}}. In the applications of our interest, missing entries are common, and we explicitly account for them by allowing for systematic model-based imputation. 

%Fourth, while the method-of-moment based approaches have been recently found to be very promising, they require the symmetric tensors to possess specific structures, which do not hold in our setting.

==> 3_algorithm.tex <==
%!TEX root = CustPrefSegment.tex
\section{Model-Based Projection Algorithm}
\label{sec:algo}

\newcommand{\xobs}{\bm{x}^{\obs}}
\newcommand{\xmis}{\bm{x}^{\mis}}
\newcommand{\projmat}{\bm{\mathrm{PSCORES}}}

In this section, we discuss our model-based projection technique for segmenting customers in more detail. For ease of describing the algorithm, we suppose that the customer labels are binary: {\em like} denoted by $+1$ and {\em dislike} denoted by $-1$. However, as we discuss later, our algorithm directly applies when the customer labels belong to any finite set. We use the terms {\em opinion} and {\em rating} interchangeably to describe the labels provided by the customers. 

We assume that the customer labels are generated according to a parametric model family $\F(\Omega) = \set{f(\bmx, \omega) \; \colon \; \omega \in \Omega}$, where $\Omega$ is the parameter space that indexes each model $f \in \F$ and $\bmx = (x_1,x_2,\ldots,x_n) \in \B := \bin^n$ is a binary vector describing the like and dislike opinion (or rating) for each item. The family $\F$ is usually chosen based on some underlying prediction problem. For instance, if the task is recommending customers new movies to watch based on their past viewing and rating behavior; the prediction problem could be to predict the rating given by the customer for the new movie. Consequently, we could choose a model family $\F$ that predicts the ratings given by customers to movies. Similarly, if the task is to recommend customers which products to buy, then we can have a model family that predicts the probability that a customer will purchase a product that is shown. We discuss specific families later in the paper.

For a population consisting of $K$ segments, there are $K$ distinct models $f_1,f_2,\dotsb,f_K$ with corresponding parameters $\omega_1,\omega_2,\dotsb, \omega_K$ so that customers in segment $k$ use model $f_k$ to generate their labels. Further, note that for a fixed $\omega \in \Omega$, $f(\cdot, \omega)$ specifies a (discrete) probability distribution on the domain $\B$ so that $\sum_{\bmy \in \B} f(\bmy, \omega) = 1$. Consequently, we frequently refer to the segment models $f_k$ as distributions on $\B$. Then, given a customer-item preference graph $\Pcal$, customer $i$ in segment $k$ generates binary vector $\bmx_i \sim f_k$ and assigns rating $x_{ij}$ for each item $j \in N(i)$ where $N(i)$ is the set of items rated by customer $i$. Let $\bm{x}_i^{\obs} \defas \left( x_{ij} \right)_{j \in N(i)}$ denote the observed rating vector from customer $i$ and define the domain $\pci = \set{(x_j)_{j \in N(i)} \; | \; \bmx \in \B}$. Given any model $f \in \F$, we define $\mi{f}(\bmy) \defas \sum_{\bm{x}_i^{\mis}} f_0(\bmy, \bm{x}_i^{\mis})$ for each $\bmy \in \pci$, where $\xmis_i$ represents the missing item ratings by customer $i$. Observe that $\mi{f}$ defines a distribution over $\pci$. Finally, let $\abs{\xiobs}$ denote the length of the vector $\xiobs$ and $\abs{N(i)}$ denote the size of the set $N(i)$, we have $\abs{\xiobs} = \abs{N(i)}$.

\subsection{Segmentation algorithm for $l$-regular preference graph $\Pcal$}
We first describe the algorithm for an $l$-regular preference graph $\Pcal$, i.e. each customer provides exactly $l$ ratings so that $\abs{\xiobs} = \abs{N(i)} = l$.
Since a priori we have no evidence for heterogeneity in the customer preferences, our algorithm begins with the hypothesis that the population is homogeneous and fits a single model $f_0 \in \F$ to the $m$ samples $\xobs_1, \xobs_2, \dotsc, \xobs_m$, that captures the preferences of the population as a whole. In other words, the algorithm assumes that each customer uses the same underlying model to generate the ratings, and consequently pools all the ratings together to estimate a single model $f_0$, which we call the {\em pooled} model. Once the pooled model is estimated, the algorithm goes back and reasons how well $f_0$ explains the observed customer ratings. Specifically, it uses the negative log-likelihood of the customer observation $\xiobs$ under the pooled model, i.e., $-\log f_0(\xiobs)$ as a measure of how well the observation $\xiobs$ is explained by the model $f_0$, so that large values of $-\log f_0(\xiobs)$ indicate that the observation $\xiobs$ is not well explained by the pooled model. Said differently, large values of $-\log f_0(\xiobs)$ mean that that customer $i$'s preferences are ``far away'' from that of the population. We denote $\proj_i = -\log f_0(\xiobs)$ as the {\em projection score} for customer $i$ since $\proj_i$ can be considered as a projection of customer $i$'s ratings under the model $f_0$ (this equivalence will become clear in section~\ref{sec:item_cat}).

%The negative log-likelihood can be interpreted in terms of cross-entropy. Specifically, because we only have observation $\bm{x}_i$ from customer $i$, we represent her using the empirical distribution $\fh_i$ on $\B$ such that:
%\begin{equation*}
%\fh_i(\bmy) = \begin{cases}
%    1, & \text{if } \bmy = \bmx_i\\
%    0, &\text{otherwise},
% \end{cases}
%\end{equation*}
%which places the entire mass on the single observation $\bmx_i$. Then the cross-entropy between $\fh_i$ and $f_0$ is given by:
%\[ H (\fh_i, f_0) = - \sum_{\bmy \in \B} \fh_i(\bmy) \log f_0(\bmy) = -\log f_0(\bmx_i) \]
%The KL-divergence of $f_0$ from $\fh_i$ is a measure of the information lost when $f_0$ is used to approximate $\fh_i$.C
%We denote $\proj_i \defas -\log f_0(\xiobs)$ as the uni-dimensional projection of customer $i$ under the model $f_0$. 
Once the projection scores are computed for each customer, we obtain the $K$ customer segments by clustering these scores using a standard distance-based clustering technique (such as the $k$-means algorithm). The process is summarized in Algorithm~\ref{alg:lreg_seg}.

\begin{algorithm}[H]
\caption{Segmentation algorithm for $l$-regular preference graph $\Pcal$}
\label{alg:lreg_seg}
\begin{algorithmic}[1]
\STATE \textbf{Input:} observed ratings $\xobs_1, \xobs_2, \ldots, \xobs_m$ where $\abs{\xiobs} = l$ for all $1\leq i \leq m$, model family $\F$, \# segments $K$
\STATE $f_0 \gets$ estimated pooled model in family $\F$
\STATE For each customer $i$ with observed rating vector $\xiobs$,
compute its projection score: \\
$\proj_i = -\log \mi{f_0}(\xiobs)$
\STATE Cluster $\set{\proj_1,\proj_2,\ldots,\proj_m}$ into $K$ groups
\STATE \textbf{Output:} Segment label $\hz_i \in \set{1,2,\ldots,K}$ for each customer $i$
\end{algorithmic}
\end{algorithm}

We make a few remarks regarding our algorithm. \ashwin{Note that Algorithm~\ref{alg:lreg_seg} does {\em not} rely on $\xiobs$ being a binary vector and can be applied even when
each $x_{ij}$ is categorical or real-valued.} The model-based clustering approaches typically posit that the population is described by the mixture distribution $g(\bmx) = \sum_{k} q_k f_k(\bmx)$, where all customers in segment $k$ are described by model $f_k \in \F$ and $q_k$ represent the size (or proportion) of segment $k$. They estimate $q_k$ and the parameters describing $f_k$, for all segments $k$. In contrast, our algorithm
% supposes that customer $i$ is described by $f_i \in \F$, but {\em does not} estimate the parameters corresponding to $f_i$. Instead, it 
fits only a single model $f_0$ from the family $\F$. The fact that we estimate only one member -- as opposed to $K$ members -- affords our algorithm two advantages: (a) {\em speed:} up to $10 \times$ faster than the standard latent class benchmark (see section~\ref{sec:simul_exp}) without the issues of initialization and convergence, typical of EM-methods; and (b) {\em flexibility:} allows for fitting models from complex parametric families $\F$, that more closely explain the customer preferences. 
% We demonstrate in Section~\ref{sec:exp} that the speed and flexibility of our algorithm allow it to outperform the benchmark methods, which are limited in their choice of $\F$ due to computational tractability.

{\em Estimating the number of segments}. In the description of the algorithm above, we assumed that the number of customer segments is provided as input. However, in practice, $K$ is often unknown and existing methods typically rely on cross-validation on information-theoretic measures like AIC, BIC etc. (see~\citep{mclachlan2004finite} for details) to estimate the number of segments. A nice feature of our algorithm is that it can automatically determine the underlying number of segments in the customer population. To achieve this, we first estimate the density of the customer projection scores $\proj_i$, using a general purpose technique like Kernel Density estimation (KDE). Having estimated the density, each ``peak'' (i.e. local maximum) in the density corresponds to values around which many of the projection scores concentrate. Consequently, we can associate each such peak with a customer segment, so that the number of segments is given by the number of peaks. The intuition is that customers who have similar preferences, will have projection scores ``close'' to each other, leading to higher concentration around certain values. The density function allows us to identify these values, and thereby the number of segments. We use this technique to estimate the number of customer segments in our real-world case studies (see sections~\ref{sec:movielens} and~\ref{sec:ebay}).

\subsection{Segmentation algorithm for general preference graph $\Pcal$} 
We now focus on the setting when the customer-item preference graph can be arbitrary, so that different customers may rate different numbers of items. The issue with directly applying Algorithm~\ref{alg:lreg_seg} in this context is that the log-likelihood of the observed rating vectors, i.e., $-\log \mi{f_0}(\xiobs)$ scales in the number of items rated by each customer, $\abs{\xiobs}$. This makes it difficult to compare the projection scores across customers. For instance, if ratings (or preferences) across items are independent under the family $\F$, then the pooled model $f_0$ is of the form $f_0(\bmx) = f_{01}(x_1) \cdot f_{02}(x_2)\dotsb f_{0n}(x_n)$, and consequently, the projection score for customer $i$ is given by $-\log \mi{f_0}(\xiobs) = -\sum_{j \in N(i)} \log f_{0j}(x_{ij})$. Therefore, the scores scale in $\abs{N(i)}$, making it difficult to compare them across customers. Similar conclusions can be drawn for more general dependency structures in $\F$. To address this issue, we consider the following normalized projection score:
\begin{equation}
\label{eq:proj_def}
	\proj_i = \frac{-\log \mi{f_0}(\xiobs)}{H(\mi{f_0})} = \frac{-\log \mi{f_0}(\bmx_i^{\obs})}{-\sum_{\bmy \in \pci} \mi{f_0}(\bmy) \log \mi{f_0}(\bmy)}.
\end{equation}
where $H(\mi{f_0})$ denotes the {\em entropy} of distribution $\mi{f_0}$.

We interpret the normalization as follows. Considering the ANOVA analogy from section~\ref{sec:setup}, suppose that we start with the hypothesis that the preferences of customer $i$ are well-explained by the pooled distribution $f_0$ and use the (negative) log-likelihood $-\log \mi{f_0}(\bmx_i^{\obs})$ as evidence to possibly reject the hypothesis. Because we only have partial observations from each customer, the log-likelihood $-\log \mi{f_0}(\bmx_i^{\obs})$ provides incomplete evidence of how well $f_0$ captures the preferences of customer $i$. To assess the confidence we can place in the evidence, we compute the entropy $H(\mi{f_0})$ of the distribution $\mi{f_0}$. Because higher values of entropy imply lower confidence, we divide the negative log-likelihood by the entropy term $H(\mi{f_0})$. Consequently, when the entropy is high, the projection score will be lower, indicating that we don't have sufficient evidence that the customer $i$'s preferences are not well-explained by $f_0$.
% One way to interpret the normalization is as follows. Our goal is to determine how well the pooled distribution $f_0$ approximates the preferences of customer $i$. But we only have partial observations. \ashwin{Therefore, we scale the log-likelihood value $-\log \mi(\bmx_i^{\obs})$ by the entropy $H(\mi)$, so that for the same negative log-likelihood value, we place a higher confidence in the approximation if $\mi$ has less uncertainty. Another way to interpret this is that we are computing distances of each customer from the pooled distribution $f_0$, and if $f_0$ has high entropy, i.e is very uncertain, then the distance should be weighed lower as opposed to when $f_0$ has low entropy.} 
With this normalization, the segmentation procedure can be summarized as in Algorithm~\ref{alg:gen_seg}.

\begin{algorithm}[H]
\caption{Segmentation algorithm for general preference graph $\Pcal$}
\label{alg:gen_seg}
\begin{algorithmic}
%\STATE \textbf{Input:} observed ratings $\bm{x}_1^{\obs}, \bm{x}_2^{\obs},\ldots, \bm{x}_m^{\obs}$, model family $\F$, \# segments $K$
\STATE {\em same as algorithm~\ref{alg:cat_full_seg} except replace step 3 with}: \\
%\STATE $f_0 \gets$ estimated pooled model from family $\F$
%\STATE For each customer $i$, let $\mi{f_0}$ denote the marginal density of $f_0$ restricted to $\pci$
%\STATE For each item $j$, $\hat{\gamma}_j \gets (d_j^+ + d_j^-)/m$
Compute projection score of customer $i$ as
\[ \proj_i = \frac{-\log \mi{f_0}(\bmx_i^{\obs})}{-\sum_{\bmy \in \pci} \mi{f_0}(\bmy) \log \mi{f_0}(\bmy)} \]
%\STATE Cluster $\set{\proj_1,\proj_2,\ldots,\proj_m}$ into $K$ segments
%\STATE \textbf{Output:} Segment label $\hz_i \in \set{1,2,\ldots,K}$ for each customer $i$
\end{algorithmic}
\end{algorithm}

\avrev{One concern with the above definition of the customer projection scores is the computation of entropy in the denominator, $H(\mi{f_0}) = -\sum_{\bmy \in \pci} \mi{f_0}(\bmy) \log \mi{f_0}(\bmy)$, which requires summing over $2^{\abs{N(i)}}$ elements in the general case when the pooled model $f_0$ can be arbitrary. To make this tractable, we focus on parametric families $\F$ with ``small'' dependencies. Specifically, if $\F$ represents the class of independent item preferences, then $f_0(\bm{x})$ has a product form $\prod_{j=1}^n f_{0j}(x_j)$, resulting in $\mi{f_0}(\bmx_i^{\obs}) = \prod_{j \in N(i)} f_{0j}(x_{ij}^{\obs})$ and $H(\mi{f_0}) = \sum_{j \in N(i)} H(f_{0j})$, both of which can be computed tractably. This idea extends to the case when $f_0$ is a product distribution over (disjoint) factors such that the maximum factor size is no larger than $n_b \ll n$. 
%In this case, $f_0$ again has a product form with each factor defined over a domain of size at most $2^{n_b}$. 
The marginalization and entropy computations now scale in $2^{n_b}$, which can be done tractably as long as $n_b$ is ``small'' enough.}
%In the cases when $n_b$ is not small, we use a lower bound approximation for the entropy, which is discussed in greater detail in Section~\ref{sec:est}. 

%More generally, we propose to approximate the marginalization and entropy computations through sampling: generate a large number of samples from $f_0$ and approximate the marginal probabilities and the entropy by computing simple averages over the samples. This procedure can be executed tractably as long as $f_0$ allows for efficient sampling. Restricted Boltzmann Machines (RBMs)~\citep{hinton2002training} comprise a large family of parametrized distributions over binary vectors that allow for efficient sampling (using Markov chain Monte Carlo (MCMC) methods). RBMs are specialized undirected graphical models that use hidden variables to model higher-order and non-linear dependencies in the data, and are one of the most popular ways of learning multivariate binary densities. They have enjoyed immense popularity recently in diverse applications such as collaborative filtering for movie recommendations~\citep{salakhutdinov2007restricted}, acoustic modeling~\citep{dahl2010phone} etc. Even though exact gradient-based maximization of the likelihood is intractable, efficient sampling-based methods have been proposed to approximate the likelihood gradient~\citep{hinton2010practical, fischer2014training} and, therefore, they provide a promising class $\F$.
%Techniques for estimating RBMs over large data sets is an active area of research in contemporary machine learning communities. Despite some existing limitations~\citep{hinton2010practical, yosinski2012visually}, RBMs offer a promising class $\F$, with tractable estimation and marginalization techniques.

\subsection{Incorporating multiple item categories}
\label{sec:item_cat}
The discussion so far focused on the case when there was no distinction between the different items, so that a single score for each customer made sense. However, in general, all items are usually not equivalent and there could exist a natural grouping or partitioning of the items. For example, in the case of movies, there exists different genres like Action, Comedy, Drama etc. or in the case of online e-commerce retailers like eBay, the items are cataloged into product categories like Clothing, Shoes, Cell Phones and Accessories etc. One can also consider a categorization of items based on clustering using some similarity measure (like Euclidean distance between feature vectors).
Items belonging to different categories should be handled differently to account for varying preferences. Here, we discuss how to extend our segmentation approach to account for multiple item categories.

Suppose that the items are partitioned into $B > 1$ categories, where $b \in \set{1,2, \ldots, B}$ represents a generic item category. Let $n_b > 0$ represent the number of items in category $b$, we have $\sum_{b=1}^B n_b = n$. We suppose that customer preferences in each category $b$ are generated according to a parametric model family $\F_b(\Omega_b) = \set{f(\bmx_b, \omega) \; \colon \; \omega \in \Omega_b}$ where $\Omega_b$ is the parameter space that indexes each model $f \in \F_b$ and $\bmx_b = (x_{b1}, x_{b2}, \ldots, x_{bn_b}) \in \B_b := \bin^{n_b}$ is a binary vector describing the like and dislike opinion for each item in category $b$. Note that we do restrict the families $\F_b$ in anyway and consequently allow for arbitrary correlations in item preferences across categories. For a heterogeneous population consisting of $K$ segments, each segment $k$ is characterized by $B$ models $(f_{k1}, f_{k2}, \ldots, f_{kB})$ where each $f_{kb} \in \F_b$. In this scenario, we observe a collection of vectors $\xiobs := (\xobs_{i1}, \xobs_{i2}, \ldots, \xobs_{iB})$ from each customer $i$ where $\xobs_{ib}$ is the rating vector for items in category $b$. Note that some of the entries in this vector can be empty if a customer $i$ does not rate any items in some category, we denote this as $\xobs_{ib} = \phi$.


\newcommand*{\horzbar}{\rule[.5ex]{2.5ex}{0.5pt}}

Given the above setup, our segmentation algorithm proceeds as follows. First, it fits a pooled model $f_{0b}$ for each item category by pooling together all customer ratings
$\xobs_{1b}, \xobs_{2b}, \ldots, \xobs_{mb}$ for items in category $b$. Then, for each customer $i$ and item category $b$, we compute a unidimensional projection $\proj_{ib}$
as in equation~\eqref{eq:proj_def} if $\xobs_{ib} \neq \phi$, otherwise we set $\proj_{ib} = \phi$. Note that these two steps are similar to the single category case. 
Now, for each customer $i$, we have a $B$-dimensional projection score vector $\bm{\proj}_i = (\proj_{i1}, \proj_{i2}, \ldots, \proj_{iB})$ where some of the entries can be missing. We can treat these vectors as rows of an $m \times B$ matrix $\projmat$ so that each row $i$ corresponds to the vector for customer $i$:
\[ 
\projmat = \begin{bmatrix}
	\proj_{11} & \proj_{12} & \dots  & \proj_{1B} \\
    \proj_{21} & \proj_{22}  & \dots  & \proj_{2B} \\
    \vdots & \vdots & \ddots & \vdots \\
    \proj_{m1} & \proj_{m2} & \dots  & \proj_{mB}
	\end{bmatrix} \]

Once we obtain this matrix, there are two possibilities: $\projmat$ is complete, i.e. contains no missing entries and $\projmat$ contains missing entries.

{\bf $\projmat$ is complete}. First, suppose that the number of categories $B \ll n$. Then, to recover the customer segments, we directly cluster the vectors $\bm{\proj}_i$ into $K$ groups using a traditional clustering algorithm like $k$-means or spectral clustering~\citep{}. Since the number of categories $B \ll n$, the dimensionality of the customer projection score vectors is ``small'' and therefore standard distance measures like Euclidean distance can be used to identify groups of similar customers. In fact, we show in section~\ref{sec:results} that for standard generative model families $\F_b$, the projection score vectors of customers in each segment concentrate around a specific vector, and as long as the underlying model parameters for different segments are distinct, the asymptotic error rate, i.e. the fraction of customers incorrectly classified, goes to zero.

However, there are cases when the number of categories $B$ can be large, in which case its not immediately clear whether traditional clustering algorithms will produce meaningful segments. Specifically, when the dimension is large, the curse of dimensionality kicks in, so that standard similarity-based measures like Euclidean distance that consider all the dimensions of the input are not able to meaningfully differentiate between similar and dissimilar objects, rendering traditional clustering algorithms ineffective (see~\cite{aggarwal2001surprising} and~\cite{steinbach2004challenges}). Since our approach relies on appropriate generative models of the data, we take inspiration from spectral projection techniques for learning mixture models that have recently been proposed in the computer science community (refer to the discussion in section~\ref{sec:related_work}). At a high level, these techniques consider the $m \times n$ sample matrix, where each row represents an independent sample from, say a Gaussian mixture model in $\Real^n$, project it onto the subspace spanned by the top $K$ principal components of the sample matrix, and then cluster the projections in the lower dimensional space. Such a projection preserves the separation between the mean vectors and at the same time ensures (tighter) concentration of the samples around the respective means. We can apply a similar technique to segment the customers based on the $m \times B$ matrix of projection scores $\projmat$. \avrev{Talk about why log-likelihood can be interpreted as normal distribution?} The algorithm is summarized below.

\begin{algorithm}[H]
\caption{Segmentation algorithm when $\projmat$ is complete}
\label{alg:cat_full_seg}
\begin{algorithmic}[1]
\STATE \textbf{Input:} observed ratings $\bm{x}_1^{\obs}, \bm{x}_2^{\obs},\ldots, \bm{x}_m^{\obs}$, model family $\F$, \# segments $K$
\STATE $f_{0b} \gets$ estimated pooled model from family $\F_b$ for all $1 \leq b \leq B$
%\STATE For each customer $i$, let $\mi{f_0}$ denote the marginal density of $f_0$ restricted to $\pci$
\STATE Compute $\proj_{ib}$ for each customer $i$ and category $b$ using step 3 of Algorithm~\ref{alg:gen_seg} whenever $\xobs_{ib} \neq \phi$ otherwise set $\proj_{ib} = \phi$
\STATE Create the $m \times B$ matrix $\projmat$ where row $i$ represents the projection vector of customer $i$, $\bm{\proj}_i = (\proj_{i1}, \proj_{i2}, \ldots, \proj_{iB})$
\STATE If $B$ is small ($B \approx K$)
\begin{itemize}
\item Cluster the rows $\set{\bm{\proj}_1, \bm{\proj}_2, \ldots, \bm{\proj}_m}$ into $K$ groups
\end{itemize}
else when $B \gg K$
\begin{itemize}
\item Project matrix $\projmat$ onto subspace spanned by top $K$ right singular vectors, i.e. compute $\projmat_r = \sum_{d=1}^K \sigma_d \bmU_d \bmV_d^T$ where $\sigma_1, \sigma_2, \ldots, \sigma_K$ are the top $K$ singular values and $\bmU_d, \bmV_d$ are the left and right singular vectors respectively
\item Cluster the rows of the matrix $\projmat_r$ into $K$ groups
\end{itemize}
\STATE \textbf{Output:} Segment label $\hz_i \in \set{1,2,\ldots,K}$ for each customer $i$
\end{algorithmic}
\end{algorithm}

{\bf $\projmat$ is incomplete}. In this scenario, the spectral projection techniques mentioned above are no longer applicable because of the missing entries. Further, to apply standard distance-based clustering techniques, we need to come up with suitable similarity measures that take into account the missing entries. However, as mentioned earlier, it is possible that two customers have no overlap in the item categories they rate, so that it can be very hard to define similarity between pairs of customers. To overcome these issues, we formulate the clustering task as a low-rank matrix decomposition (or factorization) problem, similar to that adopted in collaborative filtering applications~\citep{rennie2005fast,mnih2007probabilistic,koren2009matrix}. The intuition is that only a small number of (latent) factors influence a customer's preferences across the different categories, so that the matrix $\projmat$ consisting of projection scores is low-rank. More specifically, given the $m \times B$ matrix $\projmat$, the goal is to compute a $r$-dimensional projection $\bm{U}_i \in \Real^{r}$ for each customer $i$ and $\bm{V}_b \in \Real^r$ for each item category $b$, which optimizes the following:
\[ \min_{\bmU, \bmV} \sum \limits_{i=1}^m \sum \limits_{b=1}^B \ind[\proj_{ib} \neq \phi] \left(\proj_{ib} - \bmU_i^T\bm{V}_b \right)^2 \]
where matrices $\bm{U} \in \Real^{m \times r}$ and $\bm{V} \in B \times r$ are such that
\[ 
\bmU = \begin{bmatrix}
	\horzbar & \bmU_1^T & \horzbar\\
	\horzbar & \bmU_2^T & \horzbar \\
     & \vdots &  \\
	\horzbar & \bmU_m^T & \horzbar 
    	\end{bmatrix} 
\;\;\;\;\; \;\;\;\;\    	
	\bmV = \begin{bmatrix}
	\horzbar & \bmV_1^T & \horzbar\\
	\horzbar & \bmV_2^T & \horzbar \\
     & \vdots &  \\
	\horzbar & \bmV_B^T & \horzbar 
    	\end{bmatrix}     	
	\]
 %$\norm{\cdot}_F$ represents the Frobenius norm computed only over the {\em observed} entries of the matrix $\projmat$. 
Note that the rank $r \leq \min(m, B)$.  When the matrix $\projmat$ is complete, it can be shown~\citep{deerwester1990indexing} that the optimal matrices $\bmU^*, \bmV^*$ for the above minimization problem are given by $\bmU^* = \bmX_r \sqrt{\bm{\Sigma}_r}$ and $\bmV^* = \bmY_r \sqrt{\bm{\Sigma}_r}$ where $\projmat = \bmX \bm{\Sigma} \bmY^T$ represents the Singular Value Decomposition (SVD) of matrix $\projmat$ and $\bmX_r, \bmY_r$ denote resp. the matrices consisting of the top $r$ left and right singular vectors and $\bm{\Sigma}_r$ is the $r \times r$ diagonal matrix consisting of the top $r$ singular values. When $r = K$, observe that this exactly corresponds to the projection of $\projmat$ onto the subspace spanned by the top $r$ right singular vectors, as was used in Algorithm~\ref{alg:cat_full_seg} above. Therefore, the low-rank decomposition can be viewed as a natural generalization of the spectral projection technique, when there are missing entries in the matrix $\projmat$. However, computing the SVD when there are (many) missing entries is far more computationally challenging than the complete case, nonetheless there has been a lot of recent work to develop scalable techniques for computing low rank decompositions when the matrix is highly sparse (as in collaborative filtering applications like Netflix), see~\cite{takacs2009scalable, mazumder2010spectral} and the references therein.

In certain contexts, the representation $\bmV_b$ can be provided externally. As a concrete example, suppose that all $B$ categories are sub-categories of a larger category, for instance in the case of movies we could have sub-genres like Romantic Comedy, Dark Comedy, etc. which fall under the umbrella of Comedy movies. Suppose that customer preferences do not vary across the Comedy sub-genres. In that case, we can choose $r=1$ with $V_b = (1)$ for all item categories. Then, we can show that the projection of customer $i$ is given by:
\[ U_i = \frac{\sum_{b \in [B]} \ind[\proj_{ib} \neq \phi] \cdot \proj_{ib}}{\sum_{b \in [B]} \ind[\proj_{ib} \neq \phi]} \]
which is just the average of the projection scores across the different categories. A uni-dimensional projection score is sufficient in this scenario, since we assume that customer preferences are influenced only by the Comedy genre. In the more general case, other representations $\bm{V}$ can be provided. Once we compute the low rank decomposition, we cluster the rows using a standard distance-based clustering technique. The algorithm is specified below:

\begin{algorithm}[H]
\caption{Segmentation algorithm when $\projmat$ is incomplete}
\label{alg:cat_gen_seg}
\begin{algorithmic}
\STATE {\em same as algorithm~\ref{alg:cat_full_seg} except replace step 5 with}: 
\begin{itemize}
\item Compute rank $r$-factorization of matrix with projection scores $\projmat \approx \bm{U}\bm{V}^T$ where $\bm{U} \in \Real^{m \times r}, \bm{V} \in \Real^{B \times r}$ and $r \leq \min(m, B)$
\item Cluster rows of matrix $\bmU\bmV^T$ into $K$ groups
\end{itemize}
\end{algorithmic}
\end{algorithm}

%\subsection{Estimating the pooled distribution}
%\label{sec:est}
%
%We now discuss how we estimate the pooled distribution $f_0 \in \F$ from the data $\bmx_1^{\obs}, \bmx_2^{\obs}, \dotsc, \bmx_m^{\obs}$. The most general family $\F$ consists of all possible multivariate distributions over binary vectors of length $n$. Because such a general family of distributions is not computationally tractable, existing literature has focused on imposing constraints on the dependence structure among the binary variables. This dependence structure is popularly expressed in a graphical form through Markov networks (aka. undirected graphical models)~\citep{koller2009probabilistic} . A Markov network $\Hcal$ over a set of random variables $\bm{X} = (X_1,X_2,\ldots,X_n)$ is an undirected graph with $n$ nodes -- one for each random variable $X_i$ -- such that the edges specify {\em conditional independencies} between the random variables: if $X_i$ and $X_j$ are {\em not} connected by an edge, then they are conditionally independent given the values of all other random variables. Indeed, a Markov network allows for a succinct representation of the dependence structure for a set of random variables. The Hammersley-Clifford theorem~\citep{hammersley1971markov} states that {\em any} distribution $f(\bm{X})$ that satisfies the conditional independencies specified by a Markov network $\Hcal$, factorizes over the {\em cliques} in $\Hcal$, so long as the distribution is positive, i.e. $f(\bm{X}) > 0$ for all $\bm{X}$. More precisely, if $\Cscr$ denotes the set of all cliques in the undirected graph $\Hcal$, then we can write:
%\[ f(\bm{X}) = \frac{1}{Z} \prod_{c\in \Cscr} \phi_c(\bm{X}_c) \]
%where $\bm{X}_c$ denotes the subset of variables in clique $c$ and $\phi_c$ is a parametrized (positive) function over the state space of variables in $\bm{X}_c$. The constant $Z$ normalizes $f$ to ensure that it represents a valid distribution.
%
%We focus on dependence structures that decompose into a collection of disjoint maximal cliques. More precisely, we focus on families $\F$ that are described by Markov networks $\Hcal$ such that the distribution $f(\bm{X})$ factors as:
%\begin{equation*}
%	f(\bm{X}) = \prod_{b=1}^B \phi_b(\bm{X}_{\I_b}),
%\end{equation*}
%where $\I_1 \cupdot \I_2 \cupdot \dotsb \cupdot \I_B$ is a {\em partition} of the vertex set $\set{1,2,\ldots,n}$ into a disjoint union of maximal cliques. We say that the distribution $f$ is a product of $B$ factors with $\phi_b(\cdot)$ representing the {\em distribution} for the $b$th factor (note that we don't need the normalization constant). This disjoint factor structure is commonly used~\citep{bien2011sparse} to make high-dimensional multivariate distributions tractable. In our case, such a factor structure may be interpreted as capturing preferences of customers across different product categories, so that preferences for items are arbitrarily correlated within the same category and are uncorrelated across different categories. The popular Nested Logit choice models impose similar factor structures~\citep{train2009discrete}.
%
%With the above disjoint factor assumption, we consider two cases: the factor decomposition structure $\I_1, \I_2, \dotsc, \I_B$ is (a) known and (b) unknown. In the former case, we propose techniques to fit $f_0$ by solving the Maximum likelihood estimation problem, either exactly or approximately, to the observed data $\bmx_1^{\obs}, \bmx_2^{\obs}, \dotsc, \bmx_m^{\obs}$. In the latter case, we propose techniques to infer the graph structure $\hat{\I}_1, \hat{\I}_2, \dotsc, \hat{\I}_B$, which we then use as an input to the techniques developed for the known structure case.
%
%\subsubsection{Estimating $f_0$ when $\I_1, \I_2, \cdots, \I_B$ are known.} \label{sec:F_known} To fit $f_0$, we use the maximum likelihood estimation (MLE) technique. Each factor $\phi_b$, $1 \leq b \leq B$, is estimated separately by solving the following maximization problem:
%\begin{align}
%	&\max_{\phi_b(\bm{y}) \colon \bm{y} \in \mathcal{B}_b}\; \sum_{i \colon \I_b \subseteq N(i)} \log \phi_b(\bmx_{i, \I_b}^{\obs}) + \sum_{i \colon N(i) \cap \I_b \subset \I_b} \log\left( \sum_{\bm{z} \in \mathcal{B}_{i,b}} \phi_b(\bmx_{i, N(i) \cap \I_b}^{\obs}, \bm{z})\right) \label{eq:mle_b}\\
%	\text{ subject to } &\sum_{\bm{y} \in \mathcal{B}_b} \phi_b(\bm{y}) = 1 \text{ and } \phi_b(\bm{y}) \geq 0~\forall~\bm{y} \in \mathcal{B}_b, \nonumber
%\end{align}
%where $\mathcal{B}_b \defas \set{-1, +1}^{\abs{\I_b}}$ and $\mathcal{B}_{i,b} \defas \set{-1, +1}^{\abs{\I_b \setminus N(i)}}$. The objective of the above optimization problem is the data log-likelihood under the distribution $\phi_b$ and involves maximizing a concave function over a convex region, which can be solved efficiently, provided $\abs{\I_b}$ is ``small''. To emphasize this, we consider three nested families: (a) independent preferences; (b) small factor sizes; and (c) general factor sizes.
%
%{\em Independent preferences.} When preferences are independent across different items, it is assumed that customer $i$ is associated with parameter vector $\bm{\omega}_i = (\alpha_{i1},\alpha_{i2},\ldots,\alpha_{in})$ and for every item $j \in N(i)$, the customer rates it $+1$ with probability $\alpha_{ij}$ and $-1$ with probability $1 - \alpha_{ij}$, independently of all other items. Letting $\Omega_{\indep} \defas \set{(\omega_1, \dotsc, \omega_n) \colon 0 \leq \omega_j \leq 1~\forall~ j}$, we denote this family by $\F_{\indep}(\Omega_{\indep})$. Because of this independence assumption, it can be seen that any distribution $f \in \F_{\indep}(\Omega_{\indep})$, decomposes into $n$ factors $\phi_{j}$, $1 \leq j \leq n$, so that $B = n$ and $\I_j = \set{j}$ for all $j$. For each $j$, the optimization problem~\eqref{eq:mle_b} reduces to a convex program in a single variable $\omega_j \defas \phi_j(+1)$ with box constraints $0 \leq \omega_j \leq 1$. The optimal solution can be shown to be $\hat{\omega}_j = \frac{d_j^+}{d_j^+ + d_j^-}$, where $d_j^+ \defas \sum_{i \colon j \in N(i)} \ind[x_{ij} = +1]$ and $d_j^- \defas \sum_{i \colon j \in N(i)} \ind[x_{ij} = -1]$ respectively denote the number of likes and dislikes received by item $j$ from all the customers. We then obtain the pooled distribution:
%\begin{equation}
%	\label{eq:ind-pen}
%	f_0(x_1,x_2,\ldots,x_n) = \prod_{j=1}^n  \hat{w}_j^{\ind[x_j = +1]} {(1-\hat{w}_j)}^{\ind[x_j=-1]}
%\end{equation}
%Note that the popular binary logit and probit models are special cases of the above independent preferences model. Further, we ignore any items that have only likes or dislikes as they do not provide any discriminative information for segmenting the customers.
%
%{\em Small factor sizes.} When the factor sizes $\abs{\I_b}$ are small, we solve the convex program in~\eqref{eq:mle_b}, for each $1 \leq b \leq B$, exactly. Otherwise, we resort to approximation techniques, as described next.
%
%{\em General factor sizes.} For general factor sizes, the convex program in~\eqref{eq:mle_b} is computationally challenging to solve because of the exponential (in $\abs{\I_b}$) number of variables. The large number of variables is a result of allowing $\phi_b$ to be a general multivariate distribution over $\B_b$. Therefore, to address this computational challenge, we parametrize $\phi_b$ to belong to a general mixture family: $\F_{\mix, C}(\Omega_{\mix}) \defas \set{\sum_{c=1}^C \pi_c \left(\prod_{j=1}^n \alpha_{cj}^{\ind[x_j = +1]} {(1-\alpha_{cj})}^{\ind[x_j = -1]}\right) \colon \bm{x} \in \mathcal{B}, \left( \pi_c, \alpha_{cj} \right)_{c,j} \in \Omega_{\mix}}$, where each member is parametrized by the mixture proportions $\pi_c$, $1 \leq c \leq C$, and model parameters $0 \leq \alpha_{cj} \leq 1$, $1 \leq c \leq C$ and $1 \leq j \leq n$. In other words, $\F_{\mix}$ is the family of the mixture of $C$ independent preferences models. Note that because the binary logit model is a special case of the independent preferences model, the mixed logit model, which is known to provide arbitrarily close approximations to general multivariate distributions~\citep{train2009discrete}, is a special case of $\F_{\mix}$. With this restriction, the optimization problem~\eqref{eq:mle_b} reduces to
%\begin{align}
%	&\max_{\pi_c, \alpha_{cj}}\; \sum_{i \colon \I_b \cap N(i) \neq \varnothing} \log \left(\sum_{c=1}^C \pi_c \prod_{j \in \I_b \cap N(i)}  \alpha_{cj}^{\ind[x_{ij} = +1]} {(1-\alpha_{cj})}^{\ind[x_{ij} = -1]} \right) \label{eq:mle_b_mix}\\
%	\text{ subject to } &\sum_{c=1}^C \pi_c = 1, \pi_c \geq 0, 0 \leq \alpha_{cj} \leq 1~\forall~ 1 \leq c \leq C,1 \leq j \leq n, \nonumber
%\end{align}
%which follows from the fact that $\sum_{\bm{z} \in \mathcal{B}_{i,b}} \phi_b(\bmx_{i, N(i) \cap \I_b}^{\obs}, \bm{z}) = \sum_c \pi_c \left(\prod_{j \in \N(i) \cap \I_b} \alpha_{cj}^{\ind[x_{ij} = +1]} {(1-\alpha_{cj})}^{\ind[x_{ij} = -1]}\right)$ due to the independence assumption for each mixture component. The optimization problem~\eqref{eq:mle_b_mix} is no longer a convex program, but it can be approximately solved using the EM algorithm.
%
%\subsubsection{Estimating $f_0$ when $\I_1, \I_2, \dotsc, \I_B$ are unknown.} \label{sec:F_unknown} We now focus on the setting when the disjoint factor structure is unknown. Learning the dependence structure between a set of variables in general is a theoretically hard problem~\citep{chickering1996learning}. Existing literature provides several practical techniques~\citep{chow1968approximating,bresler2008reconstruction,ravikumar2010high} to estimate the dependency structure between discrete random variables from a set of joint observations. However, these techniques impose specific conditions on the dependency structure such as having no cycles (tree-structured), having bounded degree or only pairwise interactions.
%Dependency learning methods for Gaussian (or continuous) data include neighborhood regression~\citep{meinshausen2006high} and the graphical Lasso~\citep{friedman2008sparse,rothman2008sparse}.
%These approaches estimate a sparse inverse covariance matrix given the observations and add edges between the variables that correspond to non-zero entries in the matrix; zeros in the inverse covariance
%matrix of a multivariate Gaussian distribution indicate absence of edges in the corresponding graphical model~\citep{besag1974spatial}. Recently, it was shown that the connected components in the dependency structure recovered by estimating the inverse covariance matrix are exactly equal to the connected components in the sample {\em covariance graph} formed by thresholding the entries of
%the sample covariance matrix, under an appropriate choice of the threshold~\citep{mazumder2012exact}. Estimating the sample covariance matrix is computationally much cheaper than estimating the inverse covariance matrix and since we are only interested in recovering the disjoint factors (as opposed to estimating the exact dependency structure), we adopt the following heuristic: (i) estimate the sample correlation matrix $S$, (ii) zero-out entries in $S$ that are below an appropriately chosen threshold, and (iii) determine the connected components in the thresholded correlation matrix $S^{thresh}$ and output them as the factors. An appealing aspect about this heuristic is that the number of factor components $B$ is automatically determined from the data. 
%% The motivation behind this approach is that given a large number of customer ratings, the sample correlation matrix should reasonably approximate the true correlation matrix (since typically $m >> n$ in our setting). However, because the observed ratings come from a mixture distribution (and the number of samples is limited), there will be some spurious correlations that are captured in the sample correlation matrix $S$ and therefore, we need a thresholding step to retain the significant correlations. Finally, the connected components in the thresholded matrix correspond to the blocks in the true correlation matrix. One nice feature of this approach is that it does not require the number of factors $B$ as input and can automatically detect it from data, as long as the threshold is chosen correctly. Similar approaches have been used before for discovering functional relationships between genes~\citep{butte2000discovering} and different strategies for thresholding have been proposed~\citep{rothman2009generalized}.
%%Therefore, we adopt a heuristic that reduces the problem of estimating the disjoint factors into a problem of clustering the $n$ items. To carry out the clustering, we use the general-purpose affinity propagation (AP)~\citep{frey2007clustering} algorithm. The AP algorithm relies on pairwise similarities among the data points and finds clusters on the basis of maximizing the total similarity between data points and suitably chosen ``exemplars'' or representative data points. It automatically determines the number of clusters $B$ from the data, which is a motivating reason for choosing this algorithm. The algorithm works by exchanging real-valued messages between the data points until a high quality set of exemplars and corresponding clusters emerges.
%%In defining the pairwise similarities, we observe that our objective is to cluster highly correlated variables together. For this reason, we use pairwise sample correlations as the similarity measures. 
%Since some of the customer ratings can be missing, we compute the (Pearson) correlation coefficient for a pair of items $j$ and $j'$ as:
%%In particular, for items $j$ and $j'$, we define their similarity as the absolute value of the Pearson correlation coefficient, computed over all customers who rated {\em both} $j$ and $j'$:
%\begin{equation*}
%	s(j,j') = \frac{\sum_{i \colon j,j' \in N(i)} \left(x_{ij} - \bar{x}_{jj'} \right) \left(x_{ij'} - \bar{x}_{j'j} \right)}{\sqrt{\sum_{i \colon j,j' \in N(i)} \left( x_{ij} - \bar{x}_{jj'}\right)^2}\sqrt{\sum_{i \colon j,j' \in N(i)} \left( x_{ij'} - \bar{x}_{j'j}\right)^2}} \text{ where } \bar{x}_{jj'} = \frac{\sum_{i \colon j,j' \in N(i)} x_{ij}}{\abs{\set{i \colon j,j' \in N(i)}}}
%\end{equation*}
%For our purpose, we use a hard thresholding scheme: $S^{thresh}_{jj'} = |S_{jj'}| \ind[|S_{jj'}| > \lambda]$ for a threshold $\lambda \in (0,1)$. We do not distinguish between positive and negative correlations, since we are only interested in measuring dependence between the items. Once we obtain the partition $\hat{\I}_1, \hat{\I}_2, \dotsc, \hat{\I}_{\hat{B}}$, we provide it as an input to the techniques discussed above in Section~\ref{sec:F_known} to fit $f_0$.
%%Note that, as defined, the similarity metric is always between $0$ and $1$. We do not distinguish between positive and negative correlations and values closer to $1$ indicate higher dependencies amongst items $j$ and $j'$. We use these similarities as inputs to the AP clustering algorithm to obtain the partition $\hat{\I}_1, \hat{\I}_2, \dotsc, \hat{\I}_B$. Having obtained the partition, we provide it as an input to the techniques discussed above in Section~\ref{sec:F_known} to fit $f_0$.
%%which follows from the fact that $\sum_{\bm{z} \in \mathcal{B}_{i,b}} \phi_b(\bmx_{i, N(i) \cap \I_b}^{\obs}, \bm{z}) = \sum_c \prod_{j \in \N(i) \cap \I_b} \alpha_{cj}^{\ind[x_{ij} = +1]} {(1-\alpha_{cj})}^{\ind[x_{ij} = -1]} $ due to the independence assumption for each mixture component. The optimization problem~\eqref{eq:mle_b_mix} is no longer a convex program, but it can be approximately solved using the EM heuristic.
%%Note that, as defined, the similarity metric is always between $0$ and $1$. We do not distinguish between positive and negative correlations and values closer to $1$ indicate higher dependencies amongst items $j$ and $j'$. We use these similarities as inputs to the AP clustering algorithm to obtain the partition $\hat{\I}_1, \hat{\I}_2, \dotsc, \hat{\I}_B$. Having obtained the partition, we provide it as an input to the techniques discussed above in Section~\ref{sec:F_known} to fit $f_0$.

